Histogram of Cell Types: Deep Learning for Automated Bone Marrow Cytology

Bone marrow cytology is required to make a hematological diagnosis, influencing critical clinical decision points in hematology. However, bone marrow cytology is tedious, limited to experienced reference centers and associated with high inter-observer variability. This may lead to a delayed or incorrect diagnosis, leaving an unmet need for innovative supporting technologies. We have developed the first ever end-to-end deep learning-based technology for automated bone marrow cytology. Starting with a bone marrow aspirate digital whole slide image, our technology rapidly and automatically detects suitable regions for cytology, and subsequently identifies and classifies all bone marrow cells in each region. This collective cytomorphological information is captured in a novel representation called Histogram of Cell Types (HCT) quantifying bone marrow cell class probability distribution and acting as a cytological "patient fingerprint". The approach achieves high accuracy in region detection (0.97 accuracy and 0.99 ROC AUC), and cell detection and cell classification (0.75 mAP, 0.78 F1-score, Log-average miss rate of 0.31). HCT has potential to revolutionize hematopathology diagnostic workflows, leading to more cost-effective, accurate diagnosis and opening the door to precision medicine.

==> cite.tex <==
@article{lee2008icsh,
  title={ICSH guidelines for the standardization of bone marrow specimens and reports},
  author={Lee, S-H and Erber, WN and Porwit, A and Tomonaga, M and Peterson, LC and International Councilfor Standardization In Hematology},
  journal={International journal of laboratory hematology},
  volume={30},
  number={5},
  pages={349--364},
  year={2008},
  publisher={Wiley Online Library}
}

@article{tetu2014canadian,
  title={Canadian licensure for the use of digital pathology for routine diagnoses: one more step toward a new era of pathology practice without borders},
  author={T{\^e}tu, Bernard and Evans, Andrew},
  journal={Archives of Pathology and Laboratory Medicine},
  volume={138},
  number={3},
  pages={302--304},
  year={2014},
  publisher={the College of American Pathologists}
}

@article{pantanowitz2014american,
  title={American Telemedicine Association clinical guidelines for telepathology},
  author={Pantanowitz, Liron and Dickinson, Kim and Evans, Andrew J and Hassell, Lewis A and Henricks, Walter H and Lennerz, Jochen K and Lowe, Amanda and Parwani, Anil V and Riben, Michael and Smith, COL Daniel and others},
  journal={Journal of pathology informatics},
  volume={5},
  year={2014},
  publisher={Wolters Kluwer--Medknow Publications}
}

@article{hanna2015overview,
  title={Overview of contemporary guidelines in digital pathology: what is available in 2015 and what still needs to be addressed?},
  author={Hanna, Matthew G and Pantanowitz, Liron and Evans, Andrew J},
  journal={Journal of clinical pathology},
  volume={68},
  number={7},
  pages={499--505},
  year={2015},
  publisher={BMJ Publishing Group}
}

@article{pantanowitz2013validating,
  title={Validating whole slide imaging for diagnostic purposes in pathology: guideline from the College of American Pathologists Pathology and Laboratory Quality Center},
  author={Pantanowitz, Liron and Sinard, John H and Henricks, Walter H and Fatheree, Lisa A and Carter, Alexis B and Contis, Lydia and Beckwith, Bruce A and Evans, Andrew J and Lal, Avtar and Parwani, Anil V},
  journal={Archives of Pathology and Laboratory Medicine},
  volume={137},
  number={12},
  pages={1710--1722},
  year={2013},
  publisher={the College of American Pathologists}
}

@article{bauer2013validation,
  title={Validation of whole slide imaging for primary diagnosis in surgical pathology},
  author={Bauer, Thomas W and Schoenfield, Lynn and Slaw, Renee J and Yerian, Lisa and Sun, Zhiyuan and Henricks, Walter H},
  journal={Archives of pathology \& laboratory medicine},
  volume={137},
  number={4},
  pages={518--524},
  year={2013},
  publisher={the College of American Pathologists}
}

@article{bain2001bone,
  title={Bone marrow aspiration},
  author={Bain, BJ},
  journal={Journal of clinical pathology},
  volume={54},
  number={9},
  pages={657--663},
  year={2001},
  publisher={BMJ Publishing Group}
}

@article{arber2017initial,
  title={Initial diagnostic workup of acute leukemia: guideline from the College of American Pathologists and the American Society of Hematology},
  author={Arber, Daniel A and Borowitz, Michael J and Cessna, Melissa and Etzell, Joan and Foucar, Kathryn and Hasserjian, Robert P and Rizzo, J Douglas and Theil, Karl and Wang, Sa A and Smith, Anthony T and others},
  journal={Archives of pathology \& laboratory medicine},
  volume={141},
  number={10},
  pages={1342--1393},
  year={2017},
  publisher={the College of American Pathologists}
}

@article{dohner2017diagnosis,
  title={Diagnosis and management of AML in adults: 2017 ELN recommendations from an international expert panel},
  author={D{\"o}hner, Hartmut and Estey, Elihu and Grimwade, David and Amadori, Sergio and Appelbaum, Frederick R and B{\"u}chner, Thomas and Dombret, Herv{\'e} and Ebert, Benjamin L and Fenaux, Pierre and Larson, Richard A and others},
  journal={Blood},
  volume={129},
  number={4},
  pages={424--447},
  year={2017},
  publisher={American Society of Hematology}
}

@article{steensma2018myelodysplastic,
  title={Myelodysplastic syndromes current treatment algorithm 2018},
  author={Steensma, David P},
  journal={Blood cancer journal},
  volume={8},
  number={5},
  pages={1--7},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{sasada2018inter,
  title={Inter-observer variance and the need for standardization in the morphological classification of myelodysplastic syndrome},
  author={Sasada, Keiko and Yamamoto, Noriko and Masuda, Hiroki and Tanaka, Yoko and Ishihara, Ayako and Takamatsu, Yasushi and Yatomi, Yutaka and Katsuda, Waichiro and Sato, Issei and Matsui, Hirotaka and others},
  journal={Leukemia research},
  volume={69},
  pages={54--59},
  year={2018},
  publisher={Elsevier}
}

@article{font2013inter,
  title={Inter-observer variance with the diagnosis of myelodysplastic syndromes (MDS) following the 2008 WHO classification},
  author={Font, P and Loscertales, J and Benavente, C and Bermejo, A and Callejas, M and Garcia-Alonso, L and Garcia-Marcilla, A and Gil, S and Lopez-Rubio, M and Martin, E and others},
  journal={Annals of hematology},
  volume={92},
  number={1},
  pages={19--24},
  year={2013},
  publisher={Springer}
}

@article{font2015interobserver,
  title={Interobserver variance in myelodysplastic syndromes with less than 5\% bone marrow blasts: unilineage vs. multilineage dysplasia and reproducibility of the threshold of 2\% blasts},
  author={Font, Patricia and Loscertales, Javier and Soto, Carlos and Ricard, Pilar and Mu{\~n}oz-Novas, Carolina and Mart{\'\i}n-Clavero, Estela and L{\'o}pez-Rubio, Montserrat and Garcia-Alonso, Luis and Callejas, Marta and Bermejo, Alfredo and others},
  journal={Annals of hematology},
  volume={94},
  number={4},
  pages={565--573},
  year={2015},
  publisher={Springer}
}

@article{goasguen2014proposal,
  title={Proposal for refining the definition of dysgranulopoiesis in acute myeloid leukemia and myelodysplastic syndromes},
  author={Goasguen, Jean E and Bennett, John M and Bain, Barbara J and Brunning, Richard and Vallespi, Maria-Teresa and Tomonaga, Masao and Zini, Gina and Renault, Alain and on Morphology, The International Working Group and others},
  journal={Leukemia research},
  volume={38},
  number={4},
  pages={447--453},
  year={2014},
  publisher={Elsevier}
}

@article{senent2013reproducibility,
  title={Reproducibility of the World Health Organization 2008 criteria for myelodysplastic syndromes},
  author={Senent, Leonor and Arenillas, Leonor and Lu{\~n}o, Elisa and Ruiz, Juan C and Sanz, Guillermo and Florensa, Lourdes},
  journal={haematologica},
  volume={98},
  number={4},
  pages={568},
  year={2013},
  publisher={Ferrata Storti Foundation}
}

@article{maassen2013validation,
  title={Validation and proposals for a refinement of the WHO 2008 classification of myelodysplastic syndromes without excess of blasts},
  author={Maassen, Anna and Strupp, Corinna and Giagounidis, Aristoteles and Kuendgen, Andrea and Nachtkamp, Kathrin and Hildebrandt, Barbara and Gattermann, Norbert and Aul, Carlo and Haas, Rainer and Germing, Ulrich},
  journal={Leukemia research},
  volume={37},
  number={1},
  pages={64--70},
  year={2013},
  publisher={Elsevier}
}

@article{naqvi2011implications,
  title={Implications of discrepancy in morphologic diagnosis of myelodysplastic syndrome between referral and tertiary care centers},
  author={Naqvi, Kiran and Jabbour, Elias and Bueso-Ramos, Carlos and Pierce, Sherry and Borthakur, Gautam and Estrov, Zeev and Ravandi, Farhad and Faderl, Stefan and Kantarjian, Hagop and Garcia-Manero, Guillermo},
  journal={Blood, The Journal of the American Society of Hematology},
  volume={118},
  number={17},
  pages={4690--4693},
  year={2011},
  publisher={American Society of Hematology Washington, DC}
}

@article{ravandi2018evaluating,
  title={Evaluating measurable residual disease in acute myeloid leukemia},
  author={Ravandi, Farhad and Walter, Roland B and Freeman, Sylvie D},
  journal={Blood advances},
  volume={2},
  number={11},
  pages={1356--1366},
  year={2018},
  publisher={American Society of Hematology Washington, DC}
}

@article{grimwade2014defining,
  title={Defining minimal residual disease in acute myeloid leukemia: which platforms are ready for “prime time”?},
  author={Grimwade, David and Freeman, Sylvie D},
  journal={Blood, The Journal of the American Society of Hematology},
  volume={124},
  number={23},
  pages={3345--3355},
  year={2014},
  publisher={American Society of Hematology Washington, DC}
}

@article{radakovich2020artificial,
  title={Artificial intelligence in hematology: current challenges and opportunities},
  author={Radakovich, Nathan and Nagy, Matthew and Nazha, Aziz},
  journal={Current hematologic malignancy reports},
  volume={15},
  number={3},
  pages={203--210},
  year={2020},
  publisher={Springer}
}

@article{chang2019artificial,
  title={Artificial intelligence in pathology},
  author={Chang, Hye Yoon and Jung, Chan Kwon and Woo, Junwoo Isaac and Lee, Sanghun and Cho, Joonyoung and Kim, Sun Woo and Kwak, Tae-Yeong},
  journal={Journal of pathology and translational medicine},
  volume={53},
  number={1},
  pages={1},
  year={2019},
  publisher={Korean Society of Pathologists and Korean Society for Cytopathology}
}

@article{jordan2015machine,
  title={Machine learning: Trends, perspectives, and prospects},
  author={Jordan, Michael I and Mitchell, Tom M},
  journal={Science},
  volume={349},
  number={6245},
  pages={255--260},
  year={2015},
  publisher={American Association for the Advancement of Science}
}

@article{lecun2015deep,
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={nature},
  volume={521},
  number={7553},
  pages={436--444},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}

@article{niazi2019digital,
  title={Digital pathology and artificial intelligence},
  author={Niazi, Muhammad Khalid Khan and Parwani, Anil V and Gurcan, Metin N},
  journal={The lancet oncology},
  volume={20},
  number={5},
  pages={e253--e261},
  year={2019},
  publisher={Elsevier}
}

@article{araujo2017classification,
  title={Classification of breast cancer histology images using convolutional neural networks},
  author={Ara{\'u}jo, Teresa and Aresta, Guilherme and Castro, Eduardo and Rouco, Jos{\'e} and Aguiar, Paulo and Eloy, Catarina and Pol{\'o}nia, Ant{\'o}nio and Campilho, Aur{\'e}lio},
  journal={PloS one},
  volume={12},
  number={6},
  pages={e0177544},
  year={2017},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{dong2014computational,
  title={Computational pathology to discriminate benign from malignant intraductal proliferations of the breast},
  author={Dong, Fei and Irshad, Humayun and Oh, Eun-Yeong and Lerwill, Melinda F and Brachtel, Elena F and Jones, Nicholas C and Knoblauch, Nicholas W and Montaser-Kouhsari, Laleh and Johnson, Nicole B and Rao, Luigi KF and others},
  journal={PloS one},
  volume={9},
  number={12},
  pages={e114885},
  year={2014},
  publisher={Public Library of Science}
}

@article{golden2017deep,
  title={Deep learning algorithms for detection of lymph node metastases from breast cancer: helping artificial intelligence be seen},
  author={Golden, Jeffrey Alan},
  journal={Jama},
  volume={318},
  number={22},
  pages={2184--2186},
  year={2017},
  publisher={American Medical Association}
}

@article{bejnordi2017diagnostic,
  title={Diagnostic assessment of deep learning algorithms for detection of lymph node metastases in women with breast cancer},
  author={Bejnordi, Babak Ehteshami and Veta, Mitko and Van Diest, Paul Johannes and Van Ginneken, Bram and Karssemeijer, Nico and Litjens, Geert and Van Der Laak, Jeroen AWM and Hermsen, Meyke and Manson, Quirine F and Balkenhol, Maschenka and others},
  journal={Jama},
  volume={318},
  number={22},
  pages={2199--2210},
  year={2017},
  publisher={American Medical Association}
}

@article{mckinney2020international,
  title={International evaluation of an AI system for breast cancer screening},
  author={McKinney, Scott Mayer and Sieniek, Marcin and Godbole, Varun and Godwin, Jonathan and Antropova, Natasha and Ashrafian, Hutan and Back, Trevor and Chesus, Mary and Corrado, Greg S and Darzi, Ara and others},
  journal={Nature},
  volume={577},
  number={7788},
  pages={89--94},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{xu2017large,
  title={Large scale tissue histopathology image classification, segmentation, and visualization via deep convolutional activation features},
  author={Xu, Yan and Jia, Zhipeng and Wang, Liang-Bo and Ai, Yuqing and Zhang, Fang and Lai, Maode and Eric, I and Chang, Chao},
  journal={BMC bioinformatics},
  volume={18},
  number={1},
  pages={1--17},
  year={2017},
  publisher={BioMed Central}
}

@article{sirinukunwattana2017gland,
  title={Gland segmentation in colon histology images: The glas challenge contest},
  author={Sirinukunwattana, Korsuk and Pluim, Josien PW and Chen, Hao and Qi, Xiaojuan and Heng, Pheng-Ann and Guo, Yun Bo and Wang, Li Yang and Matuszewski, Bogdan J and Bruni, Elia and Sanchez, Urko and others},
  journal={Medical image analysis},
  volume={35},
  pages={489--502},
  year={2017},
  publisher={Elsevier}
}

@article{korbar2017deep,
  title={Deep learning for classification of colorectal polyps on whole-slide images},
  author={Korbar, Bruno and Olofson, Andrea M and Miraflor, Allen P and Nicka, Catherine M and Suriawinata, Matthew A and Torresani, Lorenzo and Suriawinata, Arief A and Hassanpour, Saeed},
  journal={Journal of pathology informatics},
  volume={8},
  year={2017},
  publisher={Wolters Kluwer--Medknow Publications}
}

@article{esteva2017dermatologist,
  title={Dermatologist-level classification of skin cancer with deep neural networks},
  author={Esteva, Andre and Kuprel, Brett and Novoa, Roberto A and Ko, Justin and Swetter, Susan M and Blau, Helen M and Thrun, Sebastian},
  journal={nature},
  volume={542},
  number={7639},
  pages={115--118},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{bulten2018unsupervised,
  title={Unsupervised prostate cancer detection on H\&E using convolutional adversarial autoencoders},
  author={Bulten, Wouter and Litjens, Geert},
  journal={arXiv preprint arXiv:1804.07098},
  year={2018}
}

@article{nguyen2010symbolic,
  title={Symbolic rule-based classification of lung cancer stages from free-text pathology reports},
  author={Nguyen, Anthony N and Lawley, Michael J and Hansen, David P and Bowman, Rayleen V and Clarke, Belinda E and Duhig, Edwina E and Colquist, Shoni},
  journal={Journal of the American Medical Informatics Association},
  volume={17},
  number={4},
  pages={440--445},
  year={2010},
  publisher={BMJ Group BMA House, Tavistock Square, London, WC1H 9JR}
}

@article{faust2019intelligent,
  title={Intelligent feature engineering and ontological mapping of brain tumour histomorphologies by deep learning},
  author={Faust, Kevin and Bala, Sudarshan and van Ommeren, Randy and Portante, Alessia and Al Qawahmed, Raniah and Djuric, Ugljesa and Diamandis, Phedias},
  journal={Nature Machine Intelligence},
  volume={1},
  number={7},
  pages={316--321},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{barker2016automated,
  title={Automated classification of brain tumor type in whole-slide digital pathology images using local representative tiles},
  author={Barker, Jocelyn and Hoogi, Assaf and Depeursinge, Adrien and Rubin, Daniel L},
  journal={Medical image analysis},
  volume={30},
  pages={60--71},
  year={2016},
  publisher={Elsevier}
}

@article{nagpal2019development,
  title={Development and validation of a deep learning algorithm for improving Gleason scoring of prostate cancer},
  author={Nagpal, Kunal and Foote, Davis and Liu, Yun and Chen, Po-Hsuan Cameron and Wulczyn, Ellery and Tan, Fraser and Olson, Niels and Smith, Jenny L and Mohtashamian, Arash and Wren, James H and others},
  journal={NPJ digital medicine},
  volume={2},
  number={1},
  pages={1--10},
  year={2019},
  publisher={Nature Publishing Group}
}

@inproceedings{masmoudi2019object,
  title={Object detection learning techniques for autonomous vehicle applications},
  author={Masmoudi, Mehdi and Ghazzai, Hakim and Frikha, Mounir and Massoud, Yehia},
  booktitle={2019 IEEE International Conference on Vehicular Electronics and Safety (ICVES)},
  pages={1--5},
  year={2019},
  organization={IEEE}
}

@inproceedings{masita2020deep,
  title={Deep Learning in Object Detection: a Review},
  author={Masita, Katleho L and Hasan, Ali N and Shongwe, Thokozani},
  booktitle={2020 International Conference on Artificial Intelligence, Big Data, Computing and Data Communication Systems (icABCD)},
  pages={1--11},
  year={2020},
  organization={IEEE}
}

@inproceedings{girshick2014rich,
  title={Rich feature hierarchies for accurate object detection and semantic segmentation},
  author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={580--587},
  year={2014}
}

@article{ren2015faster,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  journal={arXiv preprint arXiv:1506.01497},
  year={2015}
}

@inproceedings{redmongirshic,
  title={Girshic), R., \& Farhadi, A.(2016). You only loo) once: Unified, realYtime object detection},
  author={Redmon, J and Divvala, S},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 779Y788)}
}

@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={779--788},
  year={2016}
}

@article{parmentier2012assessment,
  title={Assessment of dysplastic hematopoiesis: lessons from healthy bone marrow donors},
  author={Parmentier, Stefani and Schetelig, Johannes and Lorenz, Kerstin and Kramer, Michael and Ireland, Robin and Schuler, Ulrich and Ordemann, Rainer and Rall, Gabi and Schaich, Markus and Bornh{\"a}user, Martin and others},
  journal={haematologica},
  volume={97},
  number={5},
  pages={723},
  year={2012},
  publisher={Ferrata Storti Foundation}
}

@article{chandradevan2020machine,
  title={Machine-based detection and classification for bone marrow aspirate differential counts: initial development focusing on nonneoplastic cells},
  author={Chandradevan, Ramraj and Aljudi, Ahmed A and Drumheller, Bradley R and Kunananthaseelan, Nilakshan and Amgad, Mohamed and Gutman, David A and Cooper, Lee AD and Jaye, David L},
  journal={Laboratory Investigation},
  volume={100},
  number={1},
  pages={98--109},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{bochkovskiy2020yolov4,
  title={Yolov4: Optimal speed and accuracy of object detection},
  author={Bochkovskiy, Alexey and Wang, Chien-Yao and Liao, Hong-Yuan Mark},
  journal={arXiv preprint arXiv:2004.10934},
  year={2020}
}

@inproceedings{laroca2018robust,
  title={A robust real-time automatic license plate recognition based on the YOLO detector},
  author={Laroca, Rayson and Severo, Evair and Zanlorensi, Luiz A and Oliveira, Luiz S and Gon{\c{c}}alves, Gabriel Resende and Schwartz, William Robson and Menotti, David},
  booktitle={2018 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--10},
  year={2018},
  organization={IEEE}
}

@inproceedings{ren2017novel,
  title={A novel YOLO-Based real-time people counting approach},
  author={Ren, Peiming and Fang, Wei and Djahel, Soufiene},
  booktitle={2017 international smart cities conference (ISC2)},
  pages={1--2},
  year={2017},
  organization={IEEE}
}

@inproceedings{wang2020cspnet,
  title={CSPNet: A new backbone that can enhance learning capability of CNN},
  author={Wang, Chien-Yao and Liao, Hong-Yuan Mark and Wu, Yueh-Hua and Chen, Ping-Yang and Hsieh, Jun-Wei and Yeh, I-Hau},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition workshops},
  pages={390--391},
  year={2020}
}

@article{he2015spatial,
  title={Spatial pyramid pooling in deep convolutional networks for visual recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={37},
  number={9},
  pages={1904--1916},
  year={2015},
  publisher={IEEE}
}

@inproceedings{liu2018path,
  title={Path aggregation network for instance segmentation},
  author={Liu, Shu and Qi, Lu and Qin, Haifang and Shi, Jianping and Jia, Jiaya},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={8759--8768},
  year={2018}
}

@article{redmon2018yolov3,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}

@inproceedings{zheng2020distance,
  title={Distance-IoU loss: Faster and better learning for bounding box regression},
  author={Zheng, Zhaohui and Wang, Ping and Liu, Wei and Li, Jinze and Ye, Rongguang and Ren, Dongwei},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={07},
  pages={12993--13000},
  year={2020}
}

@article{misra2019mish,
  title={Mish: A self regularized non-monotonic activation function},
  author={Misra, Diganta},
  journal={arXiv preprint arXiv:1908.08681},
  year={2019}
}

@article{ghiasi2018dropblock,
  title={Dropblock: A regularization method for convolutional networks},
  author={Ghiasi, Golnaz and Lin, Tsung-Yi and Le, Quoc V},
  journal={arXiv preprint arXiv:1810.12890},
  year={2018}
}

@article{loshchilov2016sgdr,
  title={Sgdr: Stochastic gradient descent with warm restarts},
  author={Loshchilov, Ilya and Hutter, Frank},
  journal={arXiv preprint arXiv:1608.03983},
  year={2016}
}

@inproceedings{yun2019cutmix,
  title={Cutmix: Regularization strategy to train strong classifiers with localizable features},
  author={Yun, Sangdoo and Han, Dongyoon and Oh, Seong Joon and Chun, Sanghyuk and Choe, Junsuk and Yoo, Youngjoon},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6023--6032},
  year={2019}
}

@inproceedings{huang2017densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4700--4708},
  year={2017}
}

@article{everingham2010pascal,
  title={The pascal visual object classes (voc) challenge},
  author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  journal={International journal of computer vision},
  volume={88},
  number={2},
  pages={303--338},
  year={2010},
  publisher={Springer}
}

@site{labelImg,
 title={LabelImg},
 author = {Bryan Russell, Antonio Torralba, William T. Freeman},
 year={2015},
 publisher={Computer Science and Artificial Intelligence Laboratory},
 site={https://github.com/tzutalin/labelImg}
}

@site{cellavision,
 author={Cellavision},
 title={https://www.cellavision.com/}
}

@article{settles2009active,
  title={Active learning literature survey},
  author={Settles, Burr},
  year={2009},
  publisher={University of Wisconsin-Madison Department of Computer Sciences}
}

@article{liu2019bone,
  title={Bone marrow cells detection: A technique for the microscopic image analysis},
  author={Liu, Hong and Cao, Haichao and Song, Enmin},
  journal={Journal of medical systems},
  volume={43},
  number={4},
  pages={1--14},
  year={2019},
  publisher={Springer}
}

@article{choi2017white,
  title={White blood cell differential count of maturation stages in bone marrow smear using dual-stage convolutional neural networks},
  author={Choi, Jin Woo and Ku, Yunseo and Yoo, Byeong Wook and Kim, Jung-Ah and Lee, Dong Soon and Chai, Young Jun and Kong, Hyoun-Joong and Kim, Hee Chan},
  journal={PloS one},
  volume={12},
  number={12},
  pages={e0189259},
  year={2017},
  publisher={Public Library of Science San Francisco, CA USA}
}

@misc{mogotsi2010christopher,
  title={Christopher d. manning, prabhakar raghavan, and hinrich sch{\"u}tze: Introduction to information retrieval},
  author={Mogotsi, IC},
  year={2010},
  publisher={Springer}
}

@inproceedings{rezatofighi2019generalized,
  title={Generalized intersection over union: A metric and a loss for bounding box regression},
  author={Rezatofighi, Hamid and Tsoi, Nathan and Gwak, JunYoung and Sadeghian, Amir and Reid, Ian and Savarese, Silvio},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={658--666},
  year={2019}
}

@article{abels2019computational,
  title={Computational pathology definitions, best practices, and recommendations for regulatory guidance: a white paper from the Digital Pathology Association},
  author={Abels, Esther and Pantanowitz, Liron and Aeffner, Famke and Zarella, Mark D and van der Laak, Jeroen and Bui, Marilyn M and Vemuri, Venkata NP and Parwani, Anil V and Gibbs, Jeff and Agosto-Arroyo, Emmanuel and others},
  journal={The Journal of pathology},
  volume={249},
  number={3},
  pages={286--294},
  year={2019},
  publisher={Wiley Online Library}
}

@article{louis2016computational,
  title={Computational pathology: a path ahead},
  author={Louis, David N and Feldman, Michael and Carter, Alexis B and Dighe, Anand S and Pfeifer, John D and Bry, Lynn and Almeida, Jonas S and Saltz, Joel and Braun, Jonathan and Tomaszewski, John E and others},
  journal={Archives of pathology \& laboratory medicine},
  volume={140},
  number={1},
  pages={41--50},
  year={2016},
  publisher={the College of American Pathologists}
}

@article{lujan2021dissecting,
  title={Dissecting the business case for adoption and implementation of digital pathology: A white paper from the digital pathology association},
  author={Lujan, Giovanni and Quigley, Jennifer C and Hartman, Douglas and Parwani, Anil and Roehmholdt, Brian and Van Meter, Bryan and Ardon, Orly and Hanna, Matthew G and Kelly, Dan and Sowards, Chelsea and others},
  journal={Journal of Pathology Informatics},
  volume={12},
  number={1},
  pages={17},
  year={2021},
  publisher={Medknow Publications}
}

@article{cheng2020challenges,
  title={Challenges in the Development, Deployment \& Regulation of Artificial Intelligence (AI) in Anatomical Pathology},
  author={Cheng, Jerome Y and Abel, Jacob T and Balis, Ulysses GJ and McClintock, David S and Pantanowitz, Liron},
  journal={The American Journal of Pathology},
  year={2020},
  publisher={Elsevier}
}
